CLIPasso: Semantically-Aware Object Sketching

Abstraction is at the heart of sketching due to the simple and minimal nature of line drawings. Abstraction entails identifying the essential visual properties of an object or scene, which requires semantic understanding and prior knowledge of high-level concepts. Abstract depictions are therefore challenging for artists, and even more so for machines. We present CLIPasso, an object sketching method that can achieve different levels of abstraction, guided by geometric and semantic simplifications. While sketch generation methods often rely on explicit sketch datasets for training, we utilize the remarkable ability of CLIP (Contrastive-Language-Image-Pretraining) to distill semantic concepts from sketches and images alike. We define a sketch as a set of B\'ezier curves and use a differentiable rasterizer to optimize the parameters of the curves directly with respect to a CLIP-based perceptual loss. The abstraction degree is controlled by varying the number of strokes. The generated sketches demonstrate multiple levels of abstraction while maintaining recognizability, underlying structure, and essential visual components of the subject drawn.

==> figs/large_figures_tex/abstraction_levels_figs.tex <==
\newcommand{\widthabsup}{0.1}

\begin{figure*}[ht]
\centering
\begin{tabular}{@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c|@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c}
    \midrule
    Input & 64 & 24 & 16 & Input & 64 & 24 & 16 \\
    \midrule
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/input/camel/camel.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/camel/camel_p16_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/camel/camel_p8_cp4.png} & 
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/camel/camel_p4_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/input/flamingo/flamingo.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/flamingo/flamingo_p16_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/flamingo/flamingo_p8_cp4.png} & 
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/flamingo/flamingo_p4_cp4.png} \\
    &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/camel/camel_p21_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/camel/camel_p10_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/camel/camel_p5_cp3.png} & &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/flamingo/flamingo_p21_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/flamingo/flamingo_p10_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/flamingo/flamingo_p5_cp3.png} \\
    &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/camel/camel_p32_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/camel/camel_p16_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/camel/camel_p8_cp2.png} & &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/flamingo/flamingo_p32_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/flamingo/flamingo_p16_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/flamingo/flamingo_p8_cp2.png} \\
    
    \midrule
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/input/rose/rose1.jpeg} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/rose1/rose_p16_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/rose1/rose_p8_cp4.png} & 
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/rose1/rose_p4_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/input/rose/rose0.jpeg} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/rose2/rose_p16_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/rose2/rose_p8_cp4.png} & 
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/rose2/rose_p4_cp4.png} \\
    &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/rose1/rose_p21_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/rose1/rose_p10_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/rose1/rose_p5_cp3.png} & &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/rose2/rose_p21_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/rose2/rose_p10_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/rose2/rose_p5_cp3.png} \\
    &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/rose1/rose_p32_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/rose1/rose_p16_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/rose1/rose_p8_cp2.png} & &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/rose2/rose_p32_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/rose2/rose_p16_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/rose2/rose_p8_cp2.png} \\
    
    \midrule
    \includegraphics[width=\widthabsup\linewidth]{figs/comp_berger/input/berger_woman.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/women/women_p32_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/women/women_p16_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/women/women_p8_cp4.png} & 
    \includegraphics[width=\widthabsup\linewidth]{figs/comp_objects/input/men/face_7_edge.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/men/men_p32_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/men/men_p16_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/men/men_p8_cp4.png} \\
    &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/women/women_p42_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/women/women_p21_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/women/women_p10_cp3.png} & &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/men/men_p42_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/men/men_p21_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/men/men_p10_cp3.png} \\
    &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/women/women_p64_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/women/women_p32_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/women/women_p16_cp2.png} & &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/men/men_p64_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/men/men_p32_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/men/men_p16_cp2.png} \\

\end{tabular}
 \caption{Sketches produced by our method with different styles and levels of abstraction. The columns indicate the total number of control points used to generate the sketch - 64, 24, and 16. The rows indicate the number of control points used for each stroke, which defines the style - 4, 3, and 2 control points respectively.}
\label{fig:abstraction_levels2}
\end{figure*}



\begin{figure*}[ht]
\centering
\begin{tabular}{@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c|@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c}
    \midrule
    Input & 64 & 24 & 16 & Input & 64 & 24 & 16 \\
    \midrule
    \includegraphics[width=\widthabsup\linewidth]{figs/comp_objects/input/horse/horse_416721310_08ac6a68e8.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/horse1/horse_p16_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/horse1/horse_p8_cp4.png} & 
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/horse1/horse_p4_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/input/giraffe/596728.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/giraffe/giraffe_p16_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/giraffe/giraffe_p8_cp4.png} & 
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/giraffe/giraffe_p4_cp4.png} \\
    &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/horse1/horse_p21_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/horse1/horse_p10_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/horse1/horse_p5_cp3.png} & &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/giraffe/giraffe_p21_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/giraffe/giraffe_p10_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/giraffe/giraffe_p5_cp3.png} \\
    &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/horse1/horse_p32_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/horse1/horse_p16_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/horse1/horse_p8_cp2.png} & &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/giraffe/giraffe_p32_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/giraffe/giraffe_p16_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/giraffe/giraffe_p8_cp2.png} \\
    
    \midrule
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/cat_47654/47654.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/cat_47654/cat_47654_p16_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/cat_47654/cat_47654_p8_cp4.png} & 
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/cat_47654/cat_47654_p4_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/cat_49281/49281.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/cat_49281/cat_49281_p16_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/cat_49281/cat_49281_p8_cp4.png} & 
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/cat_49281/cat_49281_p4_cp4.png} \\
    &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/cat_47654/cat_47654_p21_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/cat_47654/cat_47654_p10_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/cat_47654/cat_47654_p5_cp3.png} & &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/cat_49281/cat_49281_p21_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/cat_49281/cat_49281_p10_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/cat_49281/cat_49281_p5_cp3.png} \\
    &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/cat_47654/cat_47654_p32_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/cat_47654/cat_47654_p16_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/cat_47654/cat_47654_p8_cp2.png} & &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/cat_49281/cat_49281_p32_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/cat_49281/cat_49281_p16_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/cat_49281/cat_49281_p8_cp2.png} \\
    
    \midrule
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_580017/580017.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_580017/elephant_580017_p32_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_580017/elephant_580017_p16_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_580017/elephant_580017_p8_cp4.png} & 
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_582775/582775.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_582775/elephant_582775_p32_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_582775/elephant_582775_p16_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_582775/elephant_582775_p8_cp4.png} \\
    &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_580017/elephant_580017_p42_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_580017/elephant_580017_p21_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_580017/elephant_580017_p10_cp3.png} & &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_582775/elephant_582775_p42_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_582775/elephant_582775_p21_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_582775/elephant_582775_p10_cp3.png} \\
    &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_580017/elephant_580017_p64_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_580017/elephant_580017_p32_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_580017/elephant_580017_p16_cp2.png} & &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_582775/elephant_582775_p64_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_582775/elephant_582775_p32_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_582775/elephant_582775_p16_cp2.png} \\
    
\end{tabular}
 \caption{Sketches produced by our method with different styles and levels of abstraction. The columns indicate the total number of control points used to generate the sketch - 64, 24, and 16. The rows indicate the number of control points used for each stroke, which defines the style - 4, 3, and 2 control points respectively.}
\label{fig:abstraction_levels3}
\end{figure*}

 
\begin{figure*}[ht]
\centering
\begin{tabular}{@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c|@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c}
    \midrule
    Input & 64 & 24 & 16 & Input & 64 & 24 & 16 \\
    \midrule
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/input/horse/horse_132.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/horse2/horse_p16_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/horse2/horse_p8_cp4.png} & 
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/horse2/horse_p4_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_1096/elephant_1096.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_1096/elephant_1096_p16_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_1096/elephant_1096_p8_cp4.png} & 
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_1096/elephant_1096_p4_cp4.png} \\
    &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/horse2/horse_p21_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/horse2/horse_p10_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/horse2/horse_p5_cp3.png} & &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_1096/elephant_1096_p21_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_1096/elephant_1096_p10_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_1096/elephant_1096_p5_cp3.png} \\
    &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/horse2/horse_p32_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/horse2/horse_p16_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/horse2/horse_p8_cp2.png} & &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_1096/elephant_1096_p32_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_1096/elephant_1096_p16_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/elephant_1096/elephant_1096_p8_cp2.png} \\
    
    \midrule
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/hen/hen.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/hen/hen_p16_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/hen/hen_p8_cp4.png} & 
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/hen/hen_p4_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/pigeon/pigeon.jpeg} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/pigeon/pigeon_p16_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/pigeon/pigeon_p8_cp4.png} & 
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/pigeon/pigeon_p4_cp4.png} \\
    &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/hen/hen_p21_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/hen/hen_p10_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/hen/hen_p5_cp3.png} & &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/pigeon/pigeon_p21_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/pigeon/pigeon_p10_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/pigeon/pigeon_p5_cp3.png} \\
    &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/hen/hen_p32_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/hen/hen_p16_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/hen/hen_p8_cp2.png} & &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/pigeon/pigeon_p32_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/pigeon/pigeon_p16_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/pigeon/pigeon_p8_cp2.png} \\
    
    \midrule
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/dog_p/dog_p.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/dog_p/dog_p_p16_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/dog_p/dog_p_p8_cp4.png} & 
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/dog_p/dog_p_p4_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/dog_5323/5323.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/dog_5323/dog_5323_p32_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/dog_5323/dog_5323_p16_cp4.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/dog_5323/dog_5323_p8_cp4.png} \\
    &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/dog_p/dog_p_p21_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/dog_p/dog_p_p10_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/dog_p/dog_p_p5_cp3.png} & &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/dog_5323/dog_5323_p42_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/dog_5323/dog_5323_p21_cp3.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/dog_5323/dog_5323_p10_cp3.png} \\
    &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/dog_p/dog_p_p32_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/dog_p/dog_p_p16_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/dog_p/dog_p_p8_cp2.png} & &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/dog_5323/dog_5323_p64_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/dog_5323/dog_5323_p32_cp2.png} &
    \includegraphics[width=\widthabsup\linewidth]{figs/abstraction_levels/dog_5323/dog_5323_p16_cp2.png} \\

\end{tabular}
 \caption{Sketches produced by our method with different styles and levels of abstraction. The columns indicate the total number of control points used to generate the sketch - 64, 24, and 16. The rows indicate the number of control points used for each stroke, which defines the style - 4, 3, and 2 control points respectively.}
\label{fig:abstraction_levels4}
\end{figure*}

\newpage
\begin{figure*}[ht]
\centering
\begin{tabular}{@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c}
    \midrule
    Input & 64 & 32 & 16 & 8 \\
    
    \midrule
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/input/men/face_9_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/64/men/face_9_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/32/men/face_9_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/16/men/face_9_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/8/men/face_9_edge.png} \\
   
    
    \midrule
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/input/men/face_2_edge.png} &
    \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/64/men/face_2_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/32/men/face_2_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/16/men/face_2_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/8/men/face_2_edge.png} \\
    
    \midrule
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/input/men/face_4_edge.png} &
      \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/64/men/face_4_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/32/men/face_4_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/16/men/face_4_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/8/men/face_4_edge_p8_best.png} \\
   
    \midrule
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/input/men/face_7_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/64/men/face_7_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/32/men/face_7_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/16/men/face_7_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/8/men/face_7_edge.png} \\

    \midrule
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/input/men/face_10_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/64/men/face_10_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/32/men/face_10_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/16/men/face_10_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/8/men/face_10_edge_p8_best.png} \\
   
\end{tabular}
 \caption{Sketches of human faces produced by our method with different levels of abstraction.}
\label{fig:men_abstractions_level}
\end{figure*}

\begin{figure*}%
\centering
\begin{tabular}{@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c}
    \midrule
    Input & 64 & 32 & 16 & 8 \\
    
    \midrule
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/input/women/face_1_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/64/women/face_1_edge_64.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/32/women/face_1_edge_p32_best.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/16/women/face_1_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/8/women/face_1_edge.png} \\
   
  \midrule
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/input/women/face_3_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/64/women/face_3_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/32/women/face_3_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/16/women/face_3_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/8/women/face_3_edge.png} \\
   
  \midrule
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/input/women/face_5_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/64/women/face_5_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/32/women/face_5_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/16/women/face_5_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/8/women/face_5_edge.png} \\
   
  \midrule
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/input/women/face_6_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/64/women/face_6_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/32/women/face_6_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/16/women/face_6_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/8/women/face_6_edge.png} \\
   
  \midrule
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/input/women/face_8_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/64/women/face_8_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/32/women/face_8_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/16/women/face_8_edge.png} &
  \includegraphics[width=0.13\linewidth]{figs/abstraction_levels/8/women/face_8_edge.png} \\
   
\end{tabular}
 \caption{Sketches of human faces produced by our method with different levels of abstraction.}
\label{fig:woman_abstractions_level}
\end{figure*}


==> figs/large_figures_tex/background_gig.tex <==
\begin{figure}
\centering
\begin{tabular}{@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c}
    \midrule
    Input & Attention & 32 & 16 & 8 & Mask & 16 \\
    
    \midrule
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/input_tree.png} &
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/tree_attn.png} &
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/tree_p32.png} &
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/tree_p16.png} &
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/tree_p8_.png} &
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/tree_mask.png} &
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/tree_mask_p16.png} \\
    
    \midrule
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/input_horse.png} &
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/horse_attn.png} &
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/horse_p32.png} &
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/horse_p16.png} &
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/horse_p8_.png} &
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/horse_mask.png} &
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/horse_mask_p16.png} \\
    
    \midrule
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/input_landscape.png} &
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/landscape_attn.png} &
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/landscape_pe0p32.png} &
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/landscape_pe0p16.png} &
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/landscape_pe0p8_.png} &
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/landscape_mask.png} &
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/landscape_mask_pe0p16.png} \\
    
    \midrule
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/input_beach.png} &
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/beach_attn.png} &
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/beach_p32.png} &
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/beach_p16.png} &
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/beach_p8_.png} &
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/beach_mask.png} &
    \includegraphics[width=\widthbackground\linewidth]{figs/background_images/beach_mask_p16.png} \\
    
\end{tabular}
 \caption{Background Analysis - the first column shows the input images with background that were used for our optimization, the second column shows the extracted attention map. Columns 3, 4, and 5 show the output sketches produced by our method, using 32, 16, and 8 strokes respectively. Column 6 shows the mask produced by pretrained U2-Net, and column 7 shows the results of our method when applied on the masked images.}
\label{fig:backgroundanalysis}
\end{figure}

==> figs/large_figures_tex/cats100.tex <==
\begin{figure*}[ht]
\centering
\begin{tabular}{@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c}
   
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/46827.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/46827.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/47520.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/47520.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/47912.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/47912.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/47913.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/47913.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/47914.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/47914.png} \\
    
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/48771.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/48771.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/48798.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/48798.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/49080.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/49080.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/49335.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/49335.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/49644.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/49644.png} \\
    
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/50704.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/50704.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/50856.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/50856.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/51034.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/51034.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/52891.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/52891.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/cat.10804.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/cat.10804.png} \\
    
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/cat.1013.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/cat.1013.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/cat.10146.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/cat.10146.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/cat.10541.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/cat.10541.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/cat.10555.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/cat.10555.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/cat.10580.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/cat.10580.png} \\
    
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/50077.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/50077.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/47087.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/47087.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/47654.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/47654.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/47247.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/47247.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/51545.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/51545.png}
    \\
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/50473.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/50473.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/48360.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/48360.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/cat.10226.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/cat.10226.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/50705.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/50705.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/46358.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/46358.png} 
    \\
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/46689.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/46689.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/48997.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/48997.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/52935.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/52935.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/48175.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/48175.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/48822.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/48822.png} 
    \\
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/50512.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/50512.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/52516.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/52516.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/cat.10420.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/cat.10420.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/51145.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/51145.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/46762.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/46762.png}
    \\
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/51630.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/51630.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/cat.10754.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/cat.10754.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/47721.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/47721.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/cat.10179.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/cat.10179.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/48407.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/48407.png}
    \\
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/50059.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/50059.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/50302.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/50302.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/49862.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/49862.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/50663.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/50663.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/49526.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/49526.png}
    \\
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/48567.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/48567.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/cat.10806.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/cat.10806.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/cat.10379.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/cat.10379.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/51778.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/51778.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/273449.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/273449.png}
    \\
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/cat.10433.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/cat.10433.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/47287.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/47287.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/50328.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/50328.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/cat.10233.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/cat.10233.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/47720.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/47720.png}
    

\end{tabular}
 \caption{Sketching "in the wild": results of 100 random images of cats from SketchCOCO \cite{gao2020sketchycoco}.}
\label{fig:many_from_same_class}
\end{figure*}

\begin{figure*}[ht]
\centering
\begin{tabular}{@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c}

    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/48002.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/48002.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/47864.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/47864.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/49057.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/49057.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/48758.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/48758.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/cat.10582.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/cat.10582.png}
    \\
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/51354.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/51354.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/48163.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/48163.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/48639.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/48639.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/49093.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/49093.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/46382.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/46382.png}
    \\
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/50855.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/50855.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/cat.10608.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/cat.10608.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/cat.10218.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/cat.10218.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/52265.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/52265.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/49281.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/49281.png}
    \\
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/48217.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/48217.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/47278.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/47278.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/51180.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/51180.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/cat.10434.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/cat.10434.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/47898.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/47898.png}
    \\
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/cat.10781.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/cat.10781.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/51179.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/51179.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/49888.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/49888.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/49861.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/49861.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/cat.10225.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/cat.10225.png}
    \\
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/49860.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/49860.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/47457.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/47457.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/51424.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/51424.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/52503.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/52503.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/cat.10193.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/cat.10193.png}
    \\
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/46984.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/46984.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/cat.10568.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/cat.10568.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/cat.10755.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/cat.10755.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/48017.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/48017.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/51383.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/51383.png}
    \\
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/47521.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/47521.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/48439.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/48439.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/cat.10769.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/cat.10769.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/48604.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/48604.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/48374.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/48374.png}
    \\
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/48375.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/48375.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/51787.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/51787.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/51547.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/51547.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/49332.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/49332.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat_input/52918.png} &
    \includegraphics[width=\widthmany\linewidth]{figs/many_sketches_same_class/cat/52918.png} 
    \\
\end{tabular}
 \caption{Sketching "in the wild": results of 100 random images of cats from SketchCOCO \cite{gao2020sketchycoco}.}
\label{fig:many_from_same_class}
\end{figure*}

==> figs/large_figures_tex/classification_per_class.tex <==
\begin{figure*}[ht!]
    \centering
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{figs/missclassification_results/sketchy_coco_classification_clip.pdf} 
    \end{subfigure}
    
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{figs/missclassification_results/sketchy_coco_classification_resnet.pdf} 
    \end{subfigure}
    
    \caption{Per-class classification accuracy of the two classifiers we used in our quantitative analysis. The figure on top shows the results for CLIP ViT-B/32 and the figure below shows the results for ResNet34 classifier. Each color represent sketches by the corresponding sketch synthesis model. }
    \label{fig:sketchy_coco_detailed_classification}
\end{figure*}

==> figs/large_figures_tex/comparison_figs.tex <==


\newpage
\begin{figure*}[ht]
\centering
\begin{tabular}{@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c}
    \midrule
    Input & A & B & C & CLIPDraw & Ours16 & Ours8 \\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/teapot/teapot_1335344868_931f5c8903.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/teapot/teapot_1335344868_931f5c8903_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/teapot/teapot_1335344868_931f5c8903.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/teapot/teapot_1335344868_931f5c8903.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/teapot/teapot_1335344868_931f5c8903_.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/teapot/teapot_1335344868_931f5c8903.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/teapot/teapot_1335344868_931f5c8903.png} \\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/teapot/teapot_85059820_8efa06eb62.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/teapot/teapot_85059820_8efa06eb62_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/teapot/teapot_85059820_8efa06eb62.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/teapot/teapot_85059820_8efa06eb62.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/teapot/teapot_85059820_8efa06eb62_.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/teapot/teapot_85059820_8efa06eb62.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/teapot/teapot_85059820_8efa06eb62.png}\\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/teapot/teapot_955318500_465c78ae97.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/teapot/teapot_955318500_465c78ae97_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/teapot/teapot_955318500_465c78ae97.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/teapot/teapot_955318500_465c78ae97.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/teapot/teapot_955318500_465c78ae97_.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/teapot/teapot_955318500_465c78ae97.png} &
     \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/teapot/teapot_955318500_465c78ae97.png} \\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/teapot/teapot_1398004645_3ee0bd8ec9.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/teapot/teapot_1398004645_3ee0bd8ec9_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/teapot/teapot_1398004645_3ee0bd8ec9.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/teapot/teapot_1398004645_3ee0bd8ec9.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/teapot/teapot_1398004645_3ee0bd8ec9_.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/teapot/teapot_1398004645_3ee0bd8ec9.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/teapot/teapot_1398004645_3ee0bd8ec9.png}\\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/teapot/teapot_1666578274_e37e59835c.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/teapot/teapot_1666578274_e37e59835c_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/teapot/teapot_1666578274_e37e59835c.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/teapot/teapot_1666578274_e37e59835c.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/teapot/teapot_1666578274_e37e59835c_.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/teapot/teapot_1666578274_e37e59835c.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/teapot/teapot_1666578274_e37e59835c.png}\\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/teapot/teapot_2122130135_53917d0b70.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/teapot/teapot_2122130135_53917d0b70_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/teapot/teapot_2122130135_53917d0b70.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/teapot/teapot_2122130135_53917d0b70.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/teapot/teapot_2122130135_53917d0b70_.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/teapot/teapot_2122130135_53917d0b70.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/teapot/teapot_2122130135_53917d0b70.png}\\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/teapot/teapot_2252638111_852bafb6e8.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/teapot/teapot_2252638111_852bafb6e8_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/teapot/teapot_2252638111_852bafb6e8_def.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/teapot/teapot_2252638111_852bafb6e8_cont.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/teapot/teapot_2252638111_852bafb6e8_.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/teapot/teapot_2252638111_852bafb6e8.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/teapot/teapot_2252638111_852bafb6e8.png}\\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/teapot/teapot_2325936501_85fe00f81b.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/teapot/teapot_2325936501_85fe00f81b_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/teapot/teapot_2325936501_85fe00f81b.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/teapot/teapot_2325936501_85fe00f81b.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/teapot/teapot_2325936501_85fe00f81b_.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/teapot/teapot_2325936501_85fe00f81b.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/teapot/teapot_2325936501_85fe00f81b.png}\\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/teapot/teapot_2478804363_9929c2e43c.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/teapot/teapot_2478804363_9929c2e43c_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/teapot/teapot_2478804363_9929c2e43c.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/teapot/teapot_2478804363_9929c2e43c.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/teapot/teapot_2478804363_9929c2e43c_.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/teapot/teapot_2478804363_9929c2e43c.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/teapot/teapot_2478804363_9929c2e43c.png}\\
    
\end{tabular}
 \caption{Comparison to competitor methods on images from the "teapot" class. Left to right : (A) Kampelm{\"{u}}hler and Pinz \cite{human-like-sketches}, (B) Li et al. \cite{Deformable_Stroke}, (C) Li et al. \cite{li2019photosketching}, and CLIPDraw \cite{CLIPDraw}.}
\label{fig:teapot}
\end{figure*}


\newpage
\begin{figure*}[ht!]
\centering
\begin{tabular}{@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c}
    \midrule
    Input & A & B & C & CLIPDraw & Ours16 & Ours8 \\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/horse/horse_327021386_90ee2a7f15.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/horse/horse_327021386_90ee2a7f15_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/horse/horse_327021386_90ee2a7f15.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/horse/horse_327021386_90ee2a7f15.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/horse/horse_327021386_90ee2a7f15.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/horse/horse_327021386_90ee2a7f15.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/horse/horse_327021386_90ee2a7f15.png} \\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/horse/horse_416721310_08ac6a68e8.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/horse/horse_416721310_08ac6a68e8_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/horse/horse_416721310_08ac6a68e8.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/horse/horse_416721310_08ac6a68e8.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/horse/horse_416721310_08ac6a68e8.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/horse/horse_416721310_08ac6a68e8.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/horse/horse_416721310_08ac6a68e8.png} \\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/horse/horse_458355343_aeb34d03e8.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/horse/horse_458355343_aeb34d03e8_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/horse/horse_458355343_aeb34d03e8.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/horse/horse_458355343_aeb34d03e8.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/horse/horse_458355343_aeb34d03e8.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/horse/horse_458355343_aeb34d03e8.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/horse/horse_458355343_aeb34d03e8.png}\\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/horse/horse_500885237_8246cbd09c.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/horse/horse_500885237_8246cbd09c_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/horse/horse_500885237_8246cbd09c.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/horse/horse_500885237_8246cbd09c.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/horse/horse_500885237_8246cbd09c.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/horse/horse_500885237_8246cbd09c.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/horse/horse_500885237_8246cbd09c.png}\\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/horse/horse_1156303540_bd2d0bce80.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/horse/horse_1156303540_bd2d0bce80_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/horse/horse_1156303540_bd2d0bce80.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/horse/horse_1156303540_bd2d0bce80.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/horse/horse_1156303540_bd2d0bce80.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/horse/horse_1156303540_bd2d0bce80.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/horse/horse_1156303540_bd2d0bce80.png} \\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/horse/horse_2143679822_711e808c54.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/horse/horse_2143679822_711e808c54_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/horse/horse_2143679822_711e808c54.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/horse/horse_2143679822_711e808c54.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/horse/horse_2143679822_711e808c54.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/horse/horse_2143679822_711e808c54.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/horse/horse_2143679822_711e808c54.png} \\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/horse/horse_anacondaT_1.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/horse/horse_anacondaT_1_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/horse/horse_anacondaT_1.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/horse/horse_anacondaT_1.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/horse/horse_anacondaT_1.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/horse/horse_anacondaT_1.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/horse/horse_anacondaT_1.png}\\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/horse/horse_DraftHorse.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/horse/horse_DraftHorse_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/horse/horse_DraftHorse.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/horse/horse_DraftHorse.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/horse/horse_DraftHorse.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/horse/horse_DraftHorse.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/horse/horse_DraftHorse.png}\\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/horse/horse_endacil_zoom.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/horse/horse_endacil_zoom_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/horse/horse_endacil_zoom.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/horse/horse_endacil_zoom.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/horse/horse_endacil_zoom.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/horse/horse_endacil_zoom.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/horse/horse_endacil_zoom.png} \\
    

\end{tabular}
 \caption{Comparison to competitor methods on images from the "horse" class. Left to right : (A) Kampelm{\"{u}}hler and Pinz \cite{human-like-sketches}, (B) Li et al. \cite{Deformable_Stroke}, (C) Li et al. \cite{li2019photosketching}, and CLIPDraw \cite{CLIPDraw}.}
\label{fig:horse}
\end{figure*}


\begin{figure*}[ht!]
\centering
\begin{tabular}{@{\hskip1pt}c@{\hskip1pt}c@{\hskip1pt}c@{\hskip1pt}c@{\hskip1pt}c@{\hskip1pt}c@{\hskip1pt}c}
    \midrule
    Input & A & B & C & CLIPDraw & Ours16 & Ours8 \\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/duck/duck_161062752_cda17c415b.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/duck/duck_161062752_cda17c415b_processed.png} &
    \raisebox{.1\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/duck/duck_161062752_cda17c415b.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/duck/duck_161062752_cda17c415b.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/duck/duck_161062752_cda17c415b_.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/duck/duck_161062752_cda17c415b.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/duck/duck_161062752_cda17c415b.png} \\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/duck/duck_457972186_5282c5ee52.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/duck/duck_457972186_5282c5ee52_processed.png} &
    \raisebox{.1\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/duck/duck_457972186_5282c5ee52.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/duck/duck_457972186_5282c5ee52.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/duck/duck_457972186_5282c5ee52_.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/duck/duck_457972186_5282c5ee52.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/duck/duck_457972186_5282c5ee52.png} \\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/duck/duck_708025181_a9d35193fb.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/duck/duck_708025181_a9d35193fb_processed.png} &
    \raisebox{.1\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/duck/duck_708025181_a9d35193fb.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/duck/duck_708025181_a9d35193fb.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/duck/duck_708025181_a9d35193fb_.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/duck/duck_708025181_a9d35193fb.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/duck/duck_708025181_a9d35193fb.png}\\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/duck/duck_811374155_ef7cb42d77.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/duck/duck_811374155_ef7cb42d77_processed.png} &
    \raisebox{.1\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/duck/duck_811374155_ef7cb42d77.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/duck/duck_811374155_ef7cb42d77.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/duck/duck_811374155_ef7cb42d77_.png} & 
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/duck/duck_811374155_ef7cb42d77.png} & 
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/duck/duck_811374155_ef7cb42d77.png}\\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/duck/duck_1478554402_55dbfa0fbc.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/duck/duck_1478554402_55dbfa0fbc_processed.png} &
    \raisebox{.1\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/duck/duck_1478554402_55dbfa0fbc.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/duck/duck_1478554402_55dbfa0fbc.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/duck/duck_1478554402_55dbfa0fbc_.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/duck/duck_1478554402_55dbfa0fbc.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/duck/duck_1478554402_55dbfa0fbc.png}\\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/duck/duck_1497314383_b36e13d3e1.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/duck/duck_1497314383_b36e13d3e1_processed.png} &
    \raisebox{.1\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/duck/duck_1497314383_b36e13d3e1.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/duck/duck_1497314383_b36e13d3e1.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/duck/duck_1497314383_b36e13d3e1_.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/duck/duck_1497314383_b36e13d3e1.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/duck/duck_1497314383_b36e13d3e1.png}\\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/duck/duck_2059530817_dcbd7ba1e8.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/duck/duck_2059530817_dcbd7ba1e8_processed.png} &
    \raisebox{.1\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/duck/duck_2059530817_dcbd7ba1e8.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/duck/duck_2059530817_dcbd7ba1e8.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/duck/duck_2059530817_dcbd7ba1e8_.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/duck/duck_2059530817_dcbd7ba1e8.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/duck/duck_2059530817_dcbd7ba1e8.png}\\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/duck/duck_2626904366_1306045cca.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/duck/duck_2626904366_1306045cca_processed.png} &
    \raisebox{.1\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/duck/duck_2626904366_1306045cca.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/duck/duck_2626904366_1306045cca.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/duck/duck_2626904366_1306045cca_.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/duck/duck_2626904366_1306045cca.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/duck/duck_2626904366_1306045cca.png}\\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/duck/duck_Anas_platyrhynchos_male.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/duck/duck_Anas_platyrhynchos_male_processed.png} &
    \raisebox{.1\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/duck/duck_Anas_platyrhynchos_male.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/duck/duck_Anas_platyrhynchos_male.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/duck/duck_Anas_platyrhynchos_male_.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/duck/duck_Anas_platyrhynchos_male.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/duck/duck_Anas_platyrhynchos_male.png}\\
    
\end{tabular}
 \caption{Comparison to competitor methods on images from the "duck" class. Left to right : (A) Kampelm{\"{u}}hler and Pinz \cite{human-like-sketches}, (B) Li et al. \cite{Deformable_Stroke}, (C) Li et al. \cite{li2019photosketching}, and CLIPDraw \cite{CLIPDraw}.}
\label{fig:duck}
\end{figure*}


\newpage
\begin{figure*}[ht!]
\centering
\begin{tabular}{@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c}
    \midrule
    Input & A & B & C & CLIPDraw & Ours16 & Ours8 \\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/bicycle/bicycle_120227459_881221f172.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/bicycle/bicycle_120227459_881221f172_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/bicycle/bicycle_120227459_881221f172.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/bicycle/bicycle_120227459_881221f172.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/bicycle/bicycle_120227459_881221f172_.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/bicycle/bicycle_120227459_881221f172.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/bicycle/bicycle_120227459_881221f172.png}\\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/bicycle/bicycle_449770950_a813122ea9_o.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/bicycle/bicycle_449770950_a813122ea9_o_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/bicycle/bicycle_449770950_a813122ea9_o.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/bicycle/bicycle_449770950_a813122ea9_o.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/bicycle/bicycle_449770950_a813122ea9_o_.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/bicycle/bicycle_449770950_a813122ea9_o.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/bicycle/bicycle_449770950_a813122ea9_o.png}\\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/bicycle/bicycle_1363322386_4f0b540836.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/bicycle/bicycle_1363322386_4f0b540836_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/bicycle/bicycle_1363322386_4f0b540836.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/bicycle/bicycle_1363322386_4f0b540836.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/bicycle/bicycle_1363322386_4f0b540836_.png} & 
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/bicycle/bicycle_1363322386_4f0b540836.png} & 
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/bicycle/bicycle_1363322386_4f0b540836.png}\\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/bicycle/bicycle_2475687435_5e85c90f18.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/bicycle/bicycle_2475687435_5e85c90f18_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/bicycle/bicycle_2475687435_5e85c90f18.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/bicycle/bicycle_2475687435_5e85c90f18.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/bicycle/bicycle_2475687435_5e85c90f18_.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/bicycle/bicycle_2475687435_5e85c90f18.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/bicycle/bicycle_2475687435_5e85c90f18.png}\\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/bicycle/bicycle_2484105649_9fd4cb0001.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/bicycle/bicycle_2484105649_9fd4cb0001_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/bicycle/bicycle_2484105649_9fd4cb0001.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/bicycle/bicycle_2484105649_9fd4cb0001.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/bicycle/bicycle_2484105649_9fd4cb0001_.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/bicycle/bicycle_2484105649_9fd4cb0001.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/bicycle/bicycle_2484105649_9fd4cb0001.png}\\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/bicycle/bicycle_2520543047_e414f7f66f.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/bicycle/bicycle_2520543047_e414f7f66f_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/bicycle/bicycle_2520543047_e414f7f66f.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/bicycle/bicycle_2520543047_e414f7f66f.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/bicycle/bicycle_2520543047_e414f7f66f_.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/bicycle/bicycle_2520543047_e414f7f66f.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/bicycle/bicycle_2520543047_e414f7f66f.png}\\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/bicycle/bicycle_200855185744624_2.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/bicycle/bicycle_200855185744624_2_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/bicycle/bicycle_200855185744624_2.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/bicycle/bicycle_200855185744624_2.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/bicycle/bicycle_200855185744624_2_.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/bicycle/bicycle_200855185744624_2.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/bicycle/bicycle_200855185744624_2.png}\\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/bicycle/bicycle_N11-13_0.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/bicycle/bicycle_N11-13_0_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/bicycle/bicycle_N11-13_0.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/bicycle/bicycle_N11-13_0.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/bicycle/bicycle_N11-13_0_.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/bicycle/bicycle_N11-13_0.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/bicycle/bicycle_N11-13_0.png}\\
    
    \midrule
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/input/bicycle/bicycle_pumabike_gid_4.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/human_like/bicycle/bicycle_pumabike_gid_4_processed.png} &
    \raisebox{.2\height}{\includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/deformable/bicycle/bicycle_pumabike_gid_4.png}} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/contour/bicycle/bicycle_pumabike_gid_4.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/clipdraw/bicycle/bicycle_pumabike_gid_4_.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours/bicycle/bicycle_pumabike_gid_4.png} &
    \includegraphics[width=\widthteapot\linewidth]{figs/comp_objects/ours8/bicycle/bicycle_pumabike_gid_4.png}\\
    
    
\end{tabular}
 \caption{Comparison to competitor methods on images from the "bicycle" class. Left to right : (A) Kampelm{\"{u}}hler and Pinz \cite{human-like-sketches}, (B) Li et al. \cite{Deformable_Stroke}, (C) Li et al. \cite{li2019photosketching}, and CLIPDraw \cite{CLIPDraw}.}
\label{fig:bicycle}
\end{figure*}


\newpage
\begin{figure*}[ht!]
\centering
\begin{tabular}{@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c}
    \midrule
    Input & A & B & C & CLIPDraw & Ours \\
    
    \midrule
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/input/men/face_9_edge.png} &
    \includegraphics[width=\widthdeformfaces\linewidth]{figs/comp_objects/deformable/men/face_9_edge_refinement.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/contour/men/face_9_edge.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/virtual_sketching/men/face_9_edge_0_pred.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/clipdraw/men/face_9_edge_.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/ours32/men/face_9_edge.png} \\
    
    \midrule
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/input/men/face_2_edge.png} &
    \includegraphics[width=\widthdeformfaces\linewidth]{figs/comp_objects/deformable/men/face_2_edge_refinement.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/contour/men/face_2_edge.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/virtual_sketching/men/face_2_edge_0_pred.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/clipdraw/men/face_2_edge_.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/ours32/men/face_2_edge.png} \\
    
    \midrule
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/input/men/face_4_edge.png} &
    \includegraphics[width=\widthdeformfaces\linewidth]{figs/comp_objects/deformable/men/face_4_edge_refinement.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/contour/men/face_4_edge.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/virtual_sketching/men/face_4_edge_0_pred.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/clipdraw/men/face_4_edge_.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/ours32/men/face_4_edge.png} \\
    
    \midrule
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/input/men/face_7_edge.png} &
    \includegraphics[width=\widthdeformfaces\linewidth]{figs/comp_objects/deformable/men/face_7_edge_refinement.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/contour/men/face_7_edge.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/virtual_sketching/men/face_7_edge_0_pred.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/clipdraw/men/face_7_edge_.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/ours32/men/face_7_edge.png} \\
    
    \midrule
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/input/men/face_10_edge.png} &
    \includegraphics[width=\widthdeformfaces\linewidth]{figs/comp_objects/deformable/men/face_10_edge_refinement.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/contour/men/face_10_edge.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/virtual_sketching/men/face_10_edge_0_pred.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/clipdraw/men/face_10_edge_.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/ours32/men/face_10_edge.png} \\
    
\end{tabular}
 \caption{Comparison to competitor methods on human faces. Left to right: (A) Li et al. \cite{Deformable_Stroke}, (B) Li et al. \cite{li2019photosketching}, (C) Mo et al. \cite{mo2021virtualsketching}, and CLIPDraw \cite{CLIPDraw}.}
\label{fig:men}
\end{figure*}


\newpage
\begin{figure*}%
\centering
\begin{tabular}{@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c}
    \midrule
    Input & A & B & C & CLIPDraw & Ours \\
    
    \midrule
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/input/women/face_1_edge.png} &
    \includegraphics[width=\widthdeformfaces\linewidth]{figs/comp_objects/deformable/women/face_1_edge_refinement.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/contour/women/face_1_edge.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/virtual_sketching/women/face_1_edge_0_pred.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/clipdraw/woman/face_1_edge_.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/ours32/women/face_1_edge.png} \\
    
      \midrule
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/input/women/face_3_edge.png} &
    \includegraphics[width=\widthdeformfaces\linewidth]{figs/comp_objects/deformable/women/face_3_edge_refinement.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/contour/women/face_3_edge.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/virtual_sketching/women/face_3_edge_0_pred.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/clipdraw/woman/face_3_edge_.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/ours32/women/face_3_edge.png} \\
    
    \midrule
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/input/women/face_5_edge.png} &
    \includegraphics[width=\widthdeformfaces\linewidth]{figs/comp_objects/deformable/women/face_5_edge_refinement.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/contour/women/face_5_edge.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/virtual_sketching/women/face_5_edge_0_pred.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/clipdraw/woman/face_5_edge_.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/ours32/women/face_5_edge.png} \\
    
    \midrule
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/input/women/face_6_edge.png} &
    \includegraphics[width=\widthdeformfaces\linewidth]{figs/comp_objects/deformable/women/face_6_edge_refinement.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/contour/women/face_6_edge.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/virtual_sketching/women/face_6_edge_0_pred.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/clipdraw/woman/face_6_edge_.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/ours32/women/face_6_edge.png} \\
    
    \midrule
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/input/women/face_8_edge.png} &
    \includegraphics[width=\widthdeformfaces\linewidth]{figs/comp_objects/deformable/women/face_8_edge_refinement.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/contour/women/face_8_edge.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/virtual_sketching/women/face_8_edge_0_pred.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/clipdraw/woman/face_8_edge_.png} &
    \includegraphics[width=0.13\linewidth]{figs/comp_objects/ours32/women/face_8_edge.png} \\
    
\end{tabular}
 \caption{Comparison to competitor methods on human faces. Left to right: (A) Li et al. \cite{Deformable_Stroke}, (B) Li et al. \cite{li2019photosketching}, (C) Mo et al. \cite{mo2021virtualsketching}, and CLIPDraw \cite{CLIPDraw}.}
\label{fig:women}
\end{figure*}


==> figs/large_figures_tex/initialisation_analysis.tex <==

\begin{figure}
\centering
\begin{tabular}{@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c}
    \midrule
     & Input & Saliency & \begin{tabular}[c]{@{}c@{}}Points\\ Sampled\end{tabular} & \begin{tabular}[c]{@{}c@{}}Initial\\ Strokes\end{tabular} & Output \\
    
    \midrule
    \rotatebox{90}{\parbox[t]{\widthattn\linewidth}{\hspace*{\fill}\begin{tabular}[c]{@{}c@{}}XDoG\\ \& ViT\end{tabular}\hspace*{\fill}}} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/cat/xdog_clip/cat_10544.jpg} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/cat_update/new_attention1_xdog1_p16_seed2000_cat0_att.png} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/cat_update/new_attention1_xdog1_p16_seed2000_cat0_distribution.png} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/cat_update/new_attention1_xdog1_p16_seed2000_cat0_init.png} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/cat_update/new_attention1_xdog1_p16_seed2000_cat0.png} \\
    
    \midrule
    \rotatebox{90}{\parbox[t]{\widthattn\linewidth}{\hspace*{\fill}ViT\hspace*{\fill}}} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/cat/xdog_clip/cat_10544.jpg} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/cat_update/new_attention1_xdog0_p16_seed2000_cat0_att.png} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/cat_update/new_attention1_xdog0_p16_seed2000_cat0_distribution.png} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/cat_update/new_attention1_xdog0_p16_seed2000_cat0_init.png} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/cat_update/new_attention1_xdog0_p16_seed2000_cat0.png} \\
    
    \midrule
    \rotatebox{90}{\parbox[t]{\widthattn\linewidth}{\hspace*{\fill}Random\hspace*{\fill}}} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/cat/xdog_clip/cat_10544.jpg} &
     &
     &
     \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/cat_update/new_attention0_xdog0_p16_seed2000_cat0_init.png} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/cat_update/new_attention0_xdog0_p16_seed2000_cat0.png}
    
\end{tabular}
 \caption{Comparison of different initialization approaches.}
\label{fig:init_analysis_cat}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}{\linewidth}
        \includegraphics[width=\linewidth]{figs/initialisation_comp/cat_update/cat-fc-loss.png}
    \end{subfigure}
    
    \begin{subfigure}{\linewidth}
        \includegraphics[width=\linewidth]{figs/initialisation_comp/cat_update/cat-total-loss.png}
    \end{subfigure}
    
    \caption{Convergence comparison with different initialization approaches.}
    \label{fig:init_cat_conv}
\end{figure}

\begin{figure}
\centering
\begin{tabular}{@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c}
    \midrule
    & Input & Saliency & \begin{tabular}[c]{@{}c@{}}Points\\ Sampled\end{tabular} & \begin{tabular}[c]{@{}c@{}}Initial\\ Strokes\end{tabular} & Output \\
    
    \midrule
    \rotatebox{90}{\parbox[t]{\widthattn\linewidth}{\hspace*{\fill}\begin{tabular}[c]{@{}c@{}}XDoG\\ \& ViT\end{tabular}\hspace*{\fill}}} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/dog_update/dog.10346.png} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/dog_update/new_attention1_xdog1_p16_seed0_dog2_att.png} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/dog_update/new_attention1_xdog1_p16_seed0_dog2_distribution.png} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/dog_update/new_attention1_xdog1_p16_seed0_dog2_init.png} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/dog_update/new_attention1_xdog1_p16_seed0_dog2.png} \\
    
    \midrule
    \rotatebox{90}{\parbox[t]{\widthattn\linewidth}{\hspace*{\fill}ViT\hspace*{\fill}}} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/dog_update/dog.10346.png} &
     \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/dog_update/new_attention1_xdog0_p16_seed0_dog2_att.png} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/dog_update/new_attention1_xdog0_p16_seed0_dog2_distribution.png} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/dog_update/new_attention1_xdog0_p16_seed0_dog2_init.png} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/dog_update/new_attention1_xdog0_p16_seed0_dog2.png} \\
    
    \midrule
    \rotatebox{90}{\parbox[t]{\widthattn\linewidth}{\hspace*{\fill}Random\hspace*{\fill}}} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/dog_update/dog.10346.png} &
     &
     &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/dog_update/new_attention0_xdog0_p16_seed0_dog2_init.png} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/dog_update/new_attention0_xdog0_p16_seed0_dog2.png} \\
    
\end{tabular}
 \caption{Comparison of different initialization approaches.}
\label{fig:init_analysis_dog}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}{\linewidth}
        \includegraphics[width=\linewidth]{figs/initialisation_comp/dog_update/dog_l_semantic.png}
    \end{subfigure}
    
    \begin{subfigure}{\linewidth}
        \includegraphics[width=\linewidth]{figs/initialisation_comp/dog_update/dog_total_loss.png}
    \end{subfigure}
    
    \caption{Convergence comparison with different initialization approaches.}
    \label{fig:init_dog_conv}
\end{figure}


\begin{figure}
\centering
\begin{tabular}{@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c}
    \midrule
     & Input & Saliency & \begin{tabular}[c]{@{}c@{}}Points\\ Sampled\end{tabular} & \begin{tabular}[c]{@{}c@{}}Initial\\ Strokes\end{tabular} & Output \\
    
    \midrule
    \rotatebox{90}{\parbox[t]{\widthattn\linewidth}{\hspace*{\fill}\begin{tabular}[c]{@{}c@{}}XDoG\\ \& ViT\end{tabular}\hspace*{\fill}}} &
    \includegraphics[width=\widthattn\linewidth]{figs/user_study/input_images/women/02-19879809258_3de6bc082b_o.png} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/women_update/new_attention1_xdog1_p16_seed2000_women3_att.png} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/women_update/new_attention1_xdog1_p16_seed2000_women3_distribution.png} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/women_update/new_attention1_xdog1_p16_seed2000_women3_init.png} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/women_update/new_attention1_xdog1_p16_seed2000_women3.png} \\
    
    \midrule
    \rotatebox{90}{\parbox[t]{\widthattn\linewidth}{\hspace*{\fill}ViT\hspace*{\fill}}} &
    \includegraphics[width=\widthattn\linewidth]{figs/user_study/input_images/women/02-19879809258_3de6bc082b_o.png} &
     \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/women_update/new_attention1_xdog0_p16_seed2000_women3_att.png} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/women_update/new_attention1_xdog0_p16_seed2000_women3_distribution.png} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/women_update/new_attention1_xdog0_p16_seed2000_women3_init.png} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/women_update/new_attention1_xdog0_p16_seed2000_women3.png} \\
    
    \midrule
    
    \rotatebox{90}{\parbox[t]{\widthattn\linewidth}{\hspace*{\fill}Random\hspace*{\fill}}} &
    \includegraphics[width=\widthattn\linewidth]{figs/user_study/input_images/women/02-19879809258_3de6bc082b_o.png} &
     &
     &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/women_update/new_attention0_xdog0_p16_seed2000_women3_init.png} &
    \includegraphics[width=\widthattn\linewidth]{figs/initialisation_comp/women_update/new_attention0_xdog0_p16_seed2000_women3.png}\\
    
\end{tabular}
 \caption{Comparison of different initialization approaches.}
\label{fig:init_analysis_woman}
\end{figure}

\begin{figure}[ht]
    \centering
    \begin{subfigure}{\linewidth}
        \includegraphics[width=\linewidth]{figs/initialisation_comp/women_update/l_semantic_women.png}
    \end{subfigure}
    
    \begin{subfigure}{\linewidth}
        \includegraphics[width=\linewidth]{figs/initialisation_comp/women_update/total_loss_women.png}
    \end{subfigure}
    
    \caption{Convergence comparison with different initialization approaches.}
    \label{fig:init_woman_conv}
\end{figure}

==> figs/large_figures_tex/missclassification_result.tex <==
\newcommand{\widthmiss}{0.24}


\begin{figure}[ht]
\centering
\begin{tabular}{@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c}
    \midrule
    A & B & \begin{tabular}[c]{@{}c@{}}Human \\ Sketches\end{tabular} & Ours16 \\
    
    \midrule
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/ResNet34/human-like/airplane_7.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/ResNet34/contour/airplane_1.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/ResNet34/human-sketches/airplane_1.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/ResNet34/ours16/airplane_5.png} \\
    
    \midrule
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/ResNet34/human-like/cat_59.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/ResNet34/contour/cat_62.png} &
    &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/ResNet34/ours16/cat_68.png} \\
    
    \midrule
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/ResNet34/human-like/dog_46.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/ResNet34/contour/dog_56.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/ResNet34/human-sketches/dog_4.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/ResNet34/ours16/dog_61.png} \\
    
    \midrule
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/ResNet34/human-like/horse_36.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/ResNet34/contour/horse_39.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/ResNet34/human-sketches/horse_3.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/ResNet34/ours16/horse_48.png} \\
    
    \midrule
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/ResNet34/human-like/sheep_24.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/ResNet34/contour/sheep_35.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/ResNet34/human-sketches/sheep_2.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/ResNet34/ours16/sheep_40.png} \\
    
\end{tabular}
 \caption{ResNet34 miss-classifications on the sketches generated by different methods (A) Kampelmühler and Pinz \cite{human-like-sketches}, (B) Li et al. \cite{li2019photosketching}. The green text on each sketch shows to correct class and the red text shows the predicted class.}
\label{fig:missclassification_rn34}
\end{figure}


\begin{figure}[ht]
\centering
\begin{tabular}{@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c}
    \midrule
    A & B & \begin{tabular}[c]{@{}c@{}}Human \\ Sketches\end{tabular} & Ours16 \\
    
    \midrule
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/CLIP/human-like/airplane_1.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/CLIP/contour/airplane_1.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/CLIP/human-sketches/airplane_1.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/CLIP/ours16/airplane_8.png} \\
    
    \midrule
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/CLIP/human-like/dog_75.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/CLIP/contour/dog_58.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/CLIP/human-sketches/dog_31.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/CLIP/ours16/dog_36.png} \\
    
    \midrule
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/CLIP/human-like/giraffe_83.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/CLIP/contour/giraffe_78.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/CLIP/human-sketches/giraffe_45.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/CLIP/ours16/giraffe_42.png} \\
    
    \midrule
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/CLIP/human-like/zebra_35.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/CLIP/contour/zebra_15.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/CLIP/human-sketches/zebra_20.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/CLIP/ours16/zebra_11.png} \\
    
    \midrule
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/CLIP/human-like/sheep_51.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/CLIP/contour/sheep_37.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/CLIP/human-sketches/sheep_27.png} &
    \includegraphics[width=\widthmiss\linewidth]{figs/misclass_new/CLIP/ours16/sheep_29.png} \\
    
\end{tabular}
 \caption{CLIP ViT-B/32 miss-classifications on the sketches generated by different methods (A) Kampelmühler and Pinz \cite{human-like-sketches}, (B) Li et al. \cite{li2019photosketching}. The green text on each sketch shows to correct class and the red text show the predicted class.}
\label{fig:missclassification_clip}
\end{figure}

==> figs/large_figures_tex/user_study_samples.tex <==

\begin{figure}[h]
\centering
\begin{tabular}{@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c}
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/cat/46415.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/cat/46827.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/cat/47721.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/cat/48822.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/cat/49861.png} \\
    \midrule
    
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/horse/57325.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/horse/57524.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/horse/horse_388.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/horse/2010_002459.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/horse/horse_567.png} \\
    \midrule
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/dog/11830.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/dog/12916.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/dog/15500.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/dog/1794.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/dog/dog.10346.png} \\
    \midrule
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/elephant/581194.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/elephant/581297.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/elephant/582398.png} &
   \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/elephant/elephant_1096.png} &
   \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/elephant/elephant_1169.png} \\
    
    \midrule
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/giraffe/595433.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/giraffe/595619.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/giraffe/596099.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/giraffe/596728.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/giraffe/597769.png} \\
\end{tabular}
 \caption{The randomly sampled animals images used for the user study.}
 \vspace{-2em}
\label{fig:user_study_input_animals}
\end{figure}


\begin{figure}[h]
\centering
\begin{tabular}{@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c}
    
    \midrule
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/men/04-wikimedia.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/men/05-34783750806_954ea83724_o.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/men/06-19876234959_388a248a3e_k.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/men/13-4727365078_655e6cd0f5_o.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/men/14-pixabay-1436663.png} \\
    
    \midrule
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/women/01-12866391563_7312cae13a_o.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/women/02-19879809258_3de6bc082b_o.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/women/08-14717382472_3119d35971_o.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/women/10-2233221399_3600271088_o.png} &
    \includegraphics[width=0.18\linewidth]{figs/user_study/input_images/women/18-20356338610_54af76bcf3_k.png} \\
    

\end{tabular}
 \caption{The randomly sampled face images used for the user study.}
\label{fig:user_study_input_face}
\end{figure}

\begin{figure}[h]
\centering
\begin{tabular}{@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c}
    \midrule
     & 32  & 16 & 8 & 4 \\
    \midrule
    \rotatebox{90}{\parbox[t]{0.2\linewidth}{\hspace*{\fill}Cat\hspace*{\fill}}} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/cat0_32_sketch.png} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/cat4_16_sketch.png} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/cat3_8__sketch.png} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/cat2_4__sketch.png} \\
    \rotatebox{90}{\parbox[t]{0.2\linewidth}{\hspace*{\fill}Horse\hspace*{\fill}}} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/horse0_32_sketch.png} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/horse4_16_sketch.png} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/horse3_8__sketch.png} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/horse2_4__sketch.png} \\
    \rotatebox{90}{\parbox[t]{0.2\linewidth}{\hspace*{\fill}Dog\hspace*{\fill}}} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/dog0_32_sketch.png} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/dog4_16_sketch.png} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/dog3_8__sketch.png} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/dog2_4__sketch.png} \\
    \rotatebox{90}{\parbox[t]{0.2\linewidth}{\hspace*{\fill}Elephant\hspace*{\fill}}} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/elephant0_ha32_sketch.png} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/elephant4_ha16_sketch.png} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/elephant3_ha8__sketch.png} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/elephant2_ha4__sketch.png} \\
    \rotatebox{90}{\parbox[t]{0.2\linewidth}{\hspace*{\fill}Giraffe\hspace*{\fill}}} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/giraffe0_32_sketch.png} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/giraffe4_16_sketch.png} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/giraffe3_8__sketch.png} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/giraffe2_4__sketch.png} \\
\end{tabular}
 \caption{Sample animal sketches produced by our method, that were used in the user study.}
\label{fig:user_study_samples}
\end{figure}

\begin{figure}[h]
\centering
\begin{tabular}{@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c@{\hskip2pt}c}
    \midrule
     & 32  & 16 & 8 & 4 \\
    \midrule
    \rotatebox{90}{\parbox[t]{0.2\linewidth}{\hspace*{\fill}Man\hspace*{\fill}}} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/men4p32.png} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/men1p16.png} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/men2p8_.png} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/men3p4_.png} \\
    
    \rotatebox{90}{\parbox[t]{0.2\linewidth}{\hspace*{\fill}Woman\hspace*{\fill}}} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/women2p32.png} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/women3p16.png} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/women1p8_.png} &
    \includegraphics[width=0.2\linewidth]{figs/user_study/survey2/women0p4_.png} \\
    
\end{tabular}
 \caption{Sample face sketches produced by our method that were used in
the user study.}
\label{fig:user_study_samples_face}
\end{figure}
